Retrieval-Augmented Multilingual Keyphrase Generation with Retriever-Generator Iterative Training

Keyphrase generation is the task of automatically predicting keyphrases given a piece of long text. Despite its recent flourishing, keyphrase generation on non-English languages haven't been vastly investigated. In this paper, we call attention to a new setting named multilingual keyphrase generation and we contribute two new datasets, EcommerceMKP and AcademicMKP, covering six languages. Technically, we propose a retrieval-augmented method for multilingual keyphrase generation to mitigate the data shortage problem in non-English languages. The retrieval-augmented model leverages keyphrase annotations in English datasets to facilitate generating keyphrases in low-resource languages. Given a non-English passage, a cross-lingual dense passage retrieval module finds relevant English passages. Then the associated English keyphrases serve as external knowledge for keyphrase generation in the current language. Moreover, we develop a retriever-generator iterative training algorithm to mine pseudo parallel passage pairs to strengthen the cross-lingual passage retriever. Comprehensive experiments and ablations show that the proposed approach outperforms all baselines.

==> tab/align_percent.tex <==
% Table generated by Excel2LaTeX from sheet 'report'
\begin{table}[!t]
  \centering
  \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}[4]{*}{\#of alignment data} & \multicolumn{2}{c}{Retrieval Recall@5} & \multicolumn{2}{c}{Gerneration F1@M} \\
\cmidrule{2-5}          & R1    & RN    & G1    & GN \\
    \midrule
    2\% (1.2k) & 50.05\% & 72.38\% & 44.50 & 45.53 \\
    3\% (1.8k) & 64.46\% & 73.32\% & 45.13 & 45.66 \\
    5\% (3k) & 68.98\% & 74.31\% & 45.17 & 45.57 \\
    10\% (6k) & 73.88\% & 76.33\% & 45.52 & 45.80 \\
    \bottomrule
    \end{tabular}%
    }
  \caption{Retriever and Generator Performance Under Different Number of Available Data}
  \label{tab:align-percent}%
\end{table}%


==> tab/dataset_stat_amzn.tex <==
% Table generated by Excel2LaTeX from sheet 'report'
\begin{table}[!t]
  \centering
  \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{c|ccccccc}
    \toprule
    \multirow{0.5}{*}{Language} & \multicolumn{1}{c}{\shortstack{Train \\ Size}} & \multicolumn{1}{c}{\shortstack{Dev \\ Size}} & \multicolumn{1}{c}{\shortstack{Test \\ Size}} & \multicolumn{1}{c}{\shortstack{Passage Length \\ (Avg/Std/Mid)}} & \multicolumn{1}{c}{\shortstack{\#Keyphrases \\ (Avg/Std/Mid)}} &  \multicolumn{1}{c}{\shortstack{Absent \\ Kps\%}} \\
    \midrule
    German (DE) & 23997 & 1411  & 2825  & 157/79/141 & 10/5/8 & 57.1\% \\
    Spanish (ES) & 12222 & 718   & 1440  & 159/84/139 & 9/5/7 & 54.6\% \\
    French (FR) & 16986 & 998   & 2000  & 163/84/144 & 9/5/8 & 63.0\% \\
    Italian (IT) & 9163  & 538   & 1081  & 167/84/152 & 8/3/7 & 42.6\% \\
    Total & 62368 & 3665  & 7346  & 161/82/143 & 9/5/7  & 56.4\% \\
    \bottomrule
    \end{tabular}%
    }
  \caption{Statistics for the EcommerceKP Dataset}
  \label{tab:dataset-stat-amaz}%
\end{table}%



==> tab/dataset_stat_pub.tex <==
% Table generated by Excel2LaTeX from sheet 'report'
\begin{table}[!t]
  \centering

  \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{c|ccccccc}
    \toprule
    \multirow{0.5}{*}{Language} & \multicolumn{1}{c}{\shortstack{Train \\ Size}} & \multicolumn{1}{c}{\shortstack{Dev \\ Size}} & \multicolumn{1}{c}{\shortstack{Test \\ Size}} & \multicolumn{1}{c}{\shortstack{Passage Length \\ (Avg/Std/Mid)}} & \multicolumn{1}{c}{\shortstack{\#Keyphrases \\ (Avg/Std/Mid)}} &  \multicolumn{1}{c}{\shortstack{Absent \\ Kps\%}} \\
    \midrule
    Chinese (ZH) & 1110  & 158   & 319   & 217/48/207 & 5/1/5 & 27.2\% \\
    Korean (KO) & 774   & 110   & 222   & 115/31/111 & 4/1/4 & 37.7\% \\
    Total & 1884  & 268   & 541   & 171/57/155 & 4/1/4 & 31.3\% \\
    \bottomrule
    \end{tabular}%
    }
  \caption{Statistics for the AcademicKP Dataset}
  \label{tab:dataset-stat-pub}%
\end{table}%


==> tab/notation.tex <==
\begin{table}[]
	\centering
	\caption{
	   Notations. 
	}\label{tab:notation}
	\renewcommand{\arraystretch}{1.3} % Default value: 1
% 	\small{
	\resizebox{1.0\columnwidth}{!}{
	\begin{tabular}{cl}
    \toprule
        Symbol & Description   \\
    \midrule
        $p^{\texttt{XX}}$ & a passage in language \texttt{XX} (\texttt{XX} $\in$ \{\texttt{DE,ES,FR,IT,KO,ZH}\})    \\
        $k^{\texttt{XX}}_{i}$ & the $i$-th target keyphrase for a passage in language \texttt{XX}    \\
        $p^{\texttt{EN}}_j$ & the $j$-th retrieved passage in English    \\
        $k^{\texttt{EN}}_{j,k}$ & the associated $k$-th keyphrase for the $j$-th retrieved passage in English    \\
    \bottomrule
    \end{tabular}
    % }
    }
\end{table}
